A Modular Framework for Distributed Model Predictive Control of Nonlinear Continuous-Time Systems (GRAMPC-D)

The modular open-source framework GRAMPC-D for model predictive control of distributed systems is presented in this paper. The modular concept allows to solve optimal control problems (OCP) in a centralized and distributed fashion using the same problem description. It is tailored to computational efficiency with the focus on embedded hardware. The distributed solution is based on the Alternating Direction Method of Multipliers (ADMM) and uses the concept of neighbor approximation to enhance convergence speed. The presented framework can be accessed through Cpp and Python and also supports plug-and-play and data exchange between agents over a network.

==> img/alg_AugmLag.tex <==
\begin{algorithm}
	\caption{Augmented Lagrangian algorithm}
	\label{alg:AugmLag}
	Initialize $\vec \nu^0$, $\vec c^0$ and set $q=1$
	\begin{algorithmic}[1]
		\STATE Update $\vec u$ and $\vec x$ by solving the minimization problem
			\begin{subequations}
				\begin{align}
					\min_{\vec u} \hspace{0.2cm} & \bar J(\vec u, \vec\nu^{q-1},\vec c^{q-1}, \tau; \vec x_0) \\
					\st \hspace{0.1cm} & \vec{\dot x} = \vec f(\vec x, \vec u, \tau),\quad \vec x(0) = \vec x_0 
				\end{align}
				\label{eq:inner}
			\end{subequations}
		\STATE Update $\vec \nu$ using the steepest ascent
			\begin{align}
				\vec \nu^q =&\ \vec \nu^{q-1} + \vec c^{q-1} \vec g(\vec x^q, \vec u^q, \tau)
			\end{align}
		\STATE Update of the penalty parameter $\vec c$ 
			\begin{align}
				\vec c^q =&\ \vec \xi(\vec u^q, \vec \nu^q, \vec c^{q-1}, \tau;\vec x_0)
			\end{align}
	\end{algorithmic}
\end{algorithm}

==> img/alg_gradient.tex <==
\begin{algorithm}
	\caption{Scetch of the projected gradient method}
	\label{alg:gradient}
	Initialize $\vec u^0$, $\vec x^0$, $\vec\lambda^0$, set $q=1$
	\begin{algorithmic}[1]
		\STATE Update $\vec\lambda^q$ by backwards integration of \eqref{eq:lambda_dot}
		\STATE Compute the gradient in \eqref{eq:duH}
		\STATE Compute a step-size $\alpha^q$
		\STATE Update the controls $\vec u^q$ by applying
			\begin{align}
				\vec u^q =&\ \vec \Psi_{\vec u}\left( \vec u^{q-1} + \alpha^q \frac{\partial}{\partial_{\vec u}}H\left(\vec x^{q-1}, \vec u^{q-1}, \vec \lambda^q, \vec\nu, \vec c, \tau\right) \right) 
				\label{eq:update_u}
			\end{align}
		\STATE Update $\vec x^q$ by forwards integration of \eqref{eq:f_dot}
		\IF{A Convergence criterion is fulfilled \textbf{or} $q=q_\textrm{max}$ }
			\STATE STOP
		\ELSE
			\STATE Set $q \leftarrow q+1$
			\STATE Go to Step 1
		\ENDIF
	\end{algorithmic}
\end{algorithm}

==> src/4_0_MPC.tex <==
\section{Model predictive control}
\label{sec:MPC}

Model predictive control (\MPC) is one of the most promising modern approaches on control theory due to its capability to consider both constraints and nonlinear dynamics. The most promising concept of \MPC\ is to approximate the control task on the infinite horizon
\begin{subequations}
	\begin{align}
	\min_{\vec u} \hspace{0.2cm} & \int_{t_0}^\infty l(\vec x, \vec u, \tau) \dtau \\
	\st & \vec{\dot x} = \vec f(\vec x, \vec u, \tau),\quad \vec x(0) = \vec x_0 \\
	& \vec 0 = \vec g(\vec x, \vec u, \tau),\ \vec 0 \geq \vec h(\vec x, \vec u, \tau) \\
	& \vec u \in \left[ \vec u_\text{min},\ \vec u_\text{max} \right].
	\end{align}
\end{subequations}
using the \textit{terminal cost} $V(\vec x(T), T) \approx \int_{t_0+T}^\infty l(\vec x, \allowbreak \vec u, \tau) \dtau$ and formulating the control task in form of a finite horizon problem
\begin{subequations}
	\begin{align}
		\min_{\vec u} \hspace{0.2cm} & J(\vec u, T; \vec x_0) \\
		\st & \vec{\dot x} = \vec f(\vec x, \vec u, \tau),\quad \vec x(0) = \vec x_0 \\
		& \vec 0 = \vec g(\vec x, \vec u, \tau),\ \vec 0 \geq \vec h(\vec x, \vec u, \tau) \\
		& \vec u \in \left[ \vec u_\text{min},\ \vec u_\text{max} \right],
	\end{align}
	\label{eq:MPC_basic_idea}%
\end{subequations}
with
\begin{align}
	J(\vec u, T; \vec x_0) = V(\vec x(T), T) + \int_{t_0}^{t_0+T} l(\vec x, \vec u, \tau) \dtau
\end{align}
see e.g. \cite{bib:jadbabaie1999,bib:jadbabaie2001}. The approximation of the terminal cost can be based on an adequate control Ljapunow function(CLF), however a common approach is to use a quadratic formulation of the form $V(\vec x(T), T) = \frac{1}{2}\norm{\vec x(T)}_{\vec P}^2$ with a positive-definite matrix $\vec P$. In each time-step the OCP \eqref{eq:MPC_basic_idea} is solved. The start of the horizon $t_0$ is set to the current time $t$ and is therefore shifted as time goes by. In the following is $t_0=0$ assumed due to convenience in notation that can always be achieved by a transformation without a loss of generality. Based on this concept a suboptimal solution to \eqref{eq:MPC_basic_idea} is sufficient as long as the suboptimality decreases in each time-step. This allows the usage of performance-oriented algorithms for MPC \cite{bib:graichen2010}. Exemplary demonstrations for practical applicability can be found e.g. in \cite{bib:kapernick2013,bib:kapernick2014}. First-order methods in specific provide fast convergence to a sufficient grade of suboptimality such as the gradient algorithm implemented in the MPC-toolbox \GRAMPC\ that is used in the presented DMPC-framework. For a comprehensive overview on first-order methods see e.g. \cite{bib:ferreau2017,bib:findeisen2018}.

%\input{src/4_2_dual}

==> src/4_1_AL.tex <==
\subsection{Augmented Lagrangian algorithm}
\label{subsec:AL}

\input{img/alg_AugmLag}

The Augmented Lagrangian algorithm is introduced in this section as it is required to derive the \ADMM\ algorithm. It enables to transform a constrained OCP 
\begin{subequations}
	\begin{align}
	\min_{\vec u} \hspace{0.2cm} & J(\vec u, T; \vec x_0) \\
	\st & \vec{\dot x} = \vec f(\vec x, \vec u, \tau),\quad \vec x(0) = \vec x_0 \\
	& \vec 0 = \vec g(\vec x, \vec u, \tau),
	\end{align}
	\label{eq:MPC_basic_idea}%
\end{subequations}
with
\begin{align}
J(\vec u, T; \vec x_0) = V(\vec x(T), T) + \int_{t_0}^{t_0+T} l(\vec x, \vec u, \tau) \dtau
\end{align}
into its unconstrained dual problem, see e.g. \cite{bib:bertsekas1996}. The idea is presented in this section regarding the equality constraints in the OCP \eqref{eq:MPC_basic_idea}. Note that the same concept can be applied to inequality constraints by transforming them into equality constraints using slack variables. For the Augmented Lagrangian approach, Lagrangian multipliers $\vec \nu(\tau)\in\R^{n_g}$ and penalty parameters $\vec c(\tau)\in\R^{n_g\times n_g}$ are introduced in the expanded cost functional
\begin{align}
	\begin{split}
		\bar J(\vec u, \vec\nu, \vec c, T; \vec x_0) =&\ J(\vec u, T; \vec x_0) + \int_0^T \vec \nu^\TT \vec g(\vec x, \vec u, \tau) \\
		&\ + \frac{1}{2} \norm{ \vec g(\vec x, \vec u, \tau) }^2_{\vec c} \dtau
	\end{split}
\end{align}
which leads to the dual problem
\begin{subequations}
	\begin{align}
		\max_{\vec \nu}\min_{\vec u} \hspace{0.2cm} & \bar J(\vec u, \vec\nu, \vec c, T; \vec x_0) \\
		\st \hspace{0.1cm} & \vec{\dot x} = \vec f(\vec x, \vec u, \tau),\quad \vec x(0) = \vec x_0
	\end{align}
	\label{eq:idea_AL}%
\end{subequations}
with the dynamics encapsulated into the inner minimization problem. The dual problem can be solved by Algorithm \ref{alg:AugmLag} in an alternating direction scheme. After initializing $\vec\nu^0$ and $\vec c^0$, the updated variables $\vec u^q$ and $\vec x^q$ are calculated in Step 1 by solving the inner minimization problem \eqref{eq:inner} subject to the dynamics $\vec f$. In Step 2, the maximization with respect to $\vec\nu$ is executed using a steepest ascent approach as the extended cost functional is linear in $\vec \nu$. The penalty parameter may be updated in Step $3$ using an adequate heuristic update law $\vec\xi$. 


==> src/4_2_dual.tex <==
\subsection{Projected gradient method}

The Augmented Lagrangian algorithm is implemented inside the MPC-toolbox \GRAMPC. Regarding the minimization in Step 1 of Algorithm \ref{alg:AugmLag}, a projected gradient method is used that is shortly presented in this section. For a more detailed description, have a look into \cite{bib:englert2019} or the documentation of \GRAMPC. It is derived by formulating the dual problem
\begin{align}
	\max_{\vec \lambda} \min_{\vec u} \hspace{0.2cm} & \bar J(\vec u, \vec\nu,\vec c, T; \vec x_0) + \int_0^T \vec \lambda^\TT \left( \vec{\dot x} - \vec f(\vec x, \vec u, \tau) \right) \dtau
	\label{eq:proj_grad}%
\end{align}
corresponding to \eqref{eq:inner} with the Lagrangian multiplier $\vec \lambda(\tau)\in\R^{n_x}$. Conditions on a stationary solution can be derived by calculus of variations and are given for \eqref{eq:proj_grad} by
\begin{subequations}
	\begin{align}
		\vec{\dot x} =&\ \vec f(\vec x, \vec u, \tau) \label{eq:f_dot}\\
		\vec{\dot \lambda} =&\ -\frac{\partial}{\partial_{\vec x}}H(\vec x, \vec u, \vec \lambda, \vec\nu, \vec c, \tau) \label{eq:lambda_dot}\\
		\vec 0 =&\ \frac{\partial}{\partial_{\vec u}} H(\vec x, \vec u, \vec \lambda, \vec\nu, \vec c, \tau) \label{eq:duH}\\
		\vec x(0) =&\ \vec x_0 \\
		\vec \lambda(T) =&\ \frac{\partial}{\partial_{\vec x}} V(\vec x(T), T)
	\end{align}
	\label{eq:opt_cond}%
\end{subequations}
with the Hamiltonian 
\begin{align}
	\begin{split}
		&H(\vec x, \vec u, \vec \lambda, \vec\nu, \vec c, \tau) \\
		&\ = l(\vec x, \vec u, \tau) + \vec \lambda^\TT \vec f(\vec x, \vec u, \tau) + \vec \nu^\TT \vec g(\vec x, \vec u, \tau) + \frac{1}{2} \norm{ \vec g(\vec x, \vec u, \tau) }^2_{\vec c}.
	\end{split}
\end{align}
The boundary-value problem \eqref{eq:opt_cond} can be solved using the projected gradient method that is presented shortly in Algorithm \ref{alg:gradient}. After initializing required variables, the update of $\vec\lambda$ is computed by a backwards integration of \eqref{eq:lambda_dot}. Afterwards, the gradient of the Hamiltonian with respect to the controls from \eqref{eq:duH} and an adequate step size are evaluated in Step 2 and 3, before in Step 4 the controls are updated by applying the update law \eqref{eq:update_u} using the projection 
\begin{align}
	\vec\Psi_{\vec u}(\vec u) =&\ 
	\begin{cases}
		\vec u_\text{max} & \text{if } \vec u > \vec u_\text{max} \\
		\vec u_\text{min} & \text{if } \vec u < \vec u_\text{min} \\
		\vec u & \text{else}.
	\end{cases}
	\label{eq:projection}
\end{align}
The projection \eqref{eq:projection} enables to consider box-constraints on the controls in a time-efficient way. The states $\vec x$ are calculated last by forwards integration of the dynamics in \eqref{eq:f_dot}. This ensures that the dynamics are satisfied even for suboptimal solutions. If a convergence criterion is fulfilled or the maximum number of iterations is reached, the projected gradient algorithm stops after the forward integration. Otherwise the iteration counter is increased and the algorithm is repeated beginning from Step 1.
\input{img/alg_gradient}

==> src/6_1_interface.tex <==
\subsection{Interface}

\input{img/img_interface}

The presented DMPC-framework is meant to be used through the provided interfaces. They can be used to describe the optimal control problem, to set the optimization parameters and to start the simulation. Consequently, the simulation results can be obtained after the simulation is done. There are two interfaces prepared, a \Cpp-interface and a Python-interface as shown in Figure \ref{img:interface}. As the framework for itself is written in \Cpp\ an interface in the same language is provided. Additionally a Python-interface is generated using the Toolbox Pybind11. Pybind11 wraps \Cpp-classes and generates standalone Python-modules, which can be imported and used in Python. In the DMPC-framework, Pybind11 is used to wrap the \Cpp-interface and make it available from Python. Hence, the functionality of both interfaces is absolutely identical and the performance of the \Cpp-code is preserved if the DMPC-framework is accessed from Python. For this reason the Python-interface combines the functionalities from Python, as e.g. plotting trajectories, with the performance of \Cpp and is the recommended choice in most scenarios. To furthermore process the simulation data the possibility of printing them into a .csv-file is prepared for either interface. 

==> src/6_1_usage.tex <==
\subsection{Modular structure of the framework}

This DMPC-framework provides an interface for both \C++ and Python. The Python interface is an exact wrapper for the \C++ -Interface, so the functionality and usage is absolute identical. As the software package Pybind11 \cite{bib:pybind11} is used as a wrapper for the \C++-Code, the Python interface combines both the functionality of Python, e.g. plotting trajectories, and the performance of \C++. It can be used by importing the Python-module that is created during the build process. This module contains the whole \C++ -code and is therefore a standalone portable module of the framework.

\subsubsection{Generate an optimal control problems}

\subsubsection{Structure of the framework}



==> src/6_2_plug-and-play.tex <==
\subsection{Plug and play}
